A semi-supervised approach to message stance classification

Social media communications are becoming increasingly prevalent; some useful, some false, whether unwittingly or maliciously. An increasing number of rumours daily flood the social networks. Determining their veracity in an autonomous way is a very active and challenging field of research, with a variety of methods proposed. However, most of the models rely on determining the constituent messages' stance towards the rumour, a feature known as the "wisdom of the crowd". Although several supervised machine-learning approaches have been proposed to tackle the message stance classification problem, these have numerous shortcomings. In this paper we argue that semi-supervised learning is more effective than supervised models and use two graph-based methods to demonstrate it. This is not only in terms of classification accuracy, but equally important, in terms of speed and scalability. We use the Label Propagation and Label Spreading algorithms and run experiments on a dataset of 72 rumours and hundreds of thousands messages collected from Twitter. We compare our results on two available datasets to the state-of-the-art to demonstrate our algorithms' performance regarding accuracy, speed and scalability for real-time applications.

==> methodGP.tex <==
%!TEX root=main.tex
\subsection{Gaussian Processes}
\label{sec:method-gaussian-processes}

if space, add details of the Gaussian processes algorithm

==> new_dataset.tex <==
For the revised version of our manuscript we have addressed one of the reviewers' comments by adding to our study another Twitter dataset, namely the ``PHEME rumour scheme dataset: journalism use case''\cite{zubiaga_liakata_procter_wong sak hoi_tolmie_2016} \footnote{https://figshare.com/articles/PHEME_rumour_scheme_dataset_journalism_use_case/2068650}. This set consists of tweet conversations, collected in association with 9 breaking news stories. The conversations are organised in threads the root of which is the initiating rumour tweet, accompanied by the corresponding replies. The tweets are annotated for support, certainty and evidentiality. In order to align this dataset with the purpose of this study, we group threads by rumour. In our nomenclature there are two levels of support in this set; whether the initial tweet supports or not the rumour and whether the subsequent tweets support the initial tweet's claim. We straighten this two-step relation, by resolving the support of each tweet against the rumour, and update the annotation accordingly. For example if the initial tweet supports the rumour claim it is annotated as such. If a subsequent tweet (reply) negates the initial tweet with certainty, then it is annotated as not supporting the rumour claim.
The dataset contains $297$ threads containing $4561$ tweets, spanning $138$ rumours organised in $9$ stories. For the purpose of this study we select only the rumours containing at least $50$ tweets. The final number of rumours we are using from this dataset is therefore $23$ containing $2233$ tweets.

